Spatio-Temporal Characterization of Qubit Routing in Connectivity-Constrained Quantum Processors

Designing efficient quantum processor topologies is pivotal for advancing scalable quantum computing architectures. The communication overhead, a critical factor affecting the execution fidelity of quantum circuits, arises from inevitable qubit routing that brings interacting qubits into physical proximity by the means of serial SWAP gates to enable the direct two-qubit gate application. Characterizing the qubit movement across the processor is crucial for tailoring techniques for minimizing the SWAP gates. This work presents a comparative analysis of the resulting communication overhead among three processor topologies: star, heavy-hexagon lattice, and square lattice topologies, according to performance metrics of communication-to-computation ratio, mean qubit hotspotness, and temporal burstiness, showcasing that the square lattice layout is favourable for quantum computer architectures at a scale.

==> acknowledgement.tex <==
\section*{Acknowledgments}

Authors gratefully acknowledge funding from the European Commission through HORIZON-EIC-2022-PATHFINDEROPEN-01-101099697 (QUADRATURE) and grant HORIZON-ERC-2021-101042080 (WINC).
